UEyes: An Eye-Tracking Dataset across User Interface Types

Different types of user interfaces differ significantly in the number of elements and how they are displayed. To examine how such differences affect the way users look at UIs, we collected and analyzed a large eye-tracking-based dataset, UEyes (62 participants, 1,980 UI screenshots, near 20K eye movement sequences), covering four major UI types: webpage, desktop UI, mobile UI, and poster. Furthermore, we analyze and discuss the differences in important factors, such as color, location, and gaze direction across UI types, individual viewing strategies and potential future directions. This position paper is a derivative of our recent paper with a particular focus on the UEyes dataset.

==> 04-Analysis.tex <==




\section{Findings}
\label{sec:analysis}
With the discussion below, we examine the data related to location bias, color bias, saccade angle and amplitude, and visited vs. revisited elements, across all UI types.
\subsection{Effect of Location}
\label{sec:analysis-location}
\begin{figure*}[!ht]
    \centering
    \def\w{0.18\linewidth}
    \subfloat[All UI types]{\includegraphics[width=\w]{figures/saliency_bias/overall_bias.png}} \hfil
    \subfloat[Webpage]{\includegraphics[width=\w]{figures/saliency_bias/webpage_bias.png}} \hfil
    \subfloat[Desktop UI]{\includegraphics[width=\w]{figures/saliency_bias/desktop_bias.png}} \hfil
    \subfloat[Mobile UI]{\includegraphics[width=\w]{figures/saliency_bias/mobile_bias.png}} \hfil
    \subfloat[Poster]{\includegraphics[width=\w]{figures/saliency_bias/poster_bias.png}}
    \caption{Location bias -- the distribution of fixations over normalized screens. \REVISION{In contrast against the center bias of natural images, fixations in user-interface settings are mostly in the upper left.}}
    \Description{This figure shows 5 location bias heatmaps for the overall, webpage, desktop, mobile, and poster, respectively.}
    \label{fig:location-bias-heatmaps}
\end{figure*}
\begin{figure*}[!ht]
    \centering
    \def\w{0.18\linewidth}
    \subfloat[All UI types]{
        \begin{minipage}{\w}
            \includegraphics[width=\linewidth]{figures/plots/results/quadrants-first1s_csv_boxplot.pdf} \\[1em]
            \includegraphics[width=\linewidth]{figures/plots/results/quadrants-first3s_csv_boxplot.pdf} \\[1em]
            \includegraphics[width=\linewidth]{figures/plots/results/quadrants_csv_boxplot.pdf}
        \end{minipage}
    } \hfil
    \subfloat[Webpage]{
        \begin{minipage}{\w}
            \includegraphics[width=\linewidth]{figures/plots/results_web/quadrants-first1s_csv_boxplot.pdf} \\[1em]
            \includegraphics[width=\linewidth]{figures/plots/results_web/quadrants-first3s_csv_boxplot.pdf} \\[1em]
            \includegraphics[width=\linewidth]{figures/plots/results_web/quadrants_csv_boxplot.pdf}
        \end{minipage}
    } \hfil
    \subfloat[Desktop UI]{
        \begin{minipage}{\w}
            \includegraphics[width=\linewidth]{figures/plots/results_desktop/quadrants-first1s_csv_boxplot.pdf} \\[1em]
            \includegraphics[width=\linewidth]{figures/plots/results_desktop/quadrants-first3s_csv_boxplot.pdf} \\[1em]
            \includegraphics[width=\linewidth]{figures/plots/results_desktop/quadrants_csv_boxplot.pdf}
        \end{minipage}
    } \hfil
    \subfloat[Mobile UI]{
        \begin{minipage}{\w}
            \includegraphics[width=\linewidth]{figures/plots/results_mobile/quadrants-first1s_csv_boxplot.pdf} \\[1em]
            \includegraphics[width=\linewidth]{figures/plots/results_mobile/quadrants-first3s_csv_boxplot.pdf} \\[1em]
            \includegraphics[width=\linewidth]{figures/plots/results_mobile/quadrants_csv_boxplot.pdf}
        \end{minipage}
    } \hfil
    \subfloat[Poster]{
        \begin{minipage}{\w}
            \includegraphics[width=\linewidth]{figures/plots/results_poster/quadrants-first1s_csv_boxplot.pdf} \\[1em]
            \includegraphics[width=\linewidth]{figures/plots/results_poster/quadrants-first3s_csv_boxplot.pdf} \\[1em]
            \includegraphics[width=\linewidth]{figures/plots/results_poster/quadrants_csv_boxplot.pdf}
        \end{minipage}
    }
    \caption{Location bias -- fixations' distribution by quadrant. \REVISION{The upper-left quadrant tends to attract more fixations than other quadrants, across all UI types.}}
    \Description{This figure shows the quadrant distribution of fixations for the overall, webpage, desktop, mobile, and poster up to 1 second, 3 seconds, and 7 seconds, respectively.}
    \label{fig:location-bias-quadrants}
\end{figure*}
\autoref{fig:location-bias-heatmaps} shows the location bias for each of the UI types, and \autoref{fig:location-bias-quadrants} displays the corresponding distribution of fixations by quadrant.
We computed the location bias by normalizing the saliency distribution relative to the individual UI image's size and then aggregating all the UI saliency results associated with each UI type. 
Overall, in contrast against the recognized center bias with natural images~\cite{bruce2005saliency},  we noticed that the upper-left quadrant of all UI types tends to attract more fixations than the other quadrants. This general result indicates that participants paid more attention to the upper-left portion of the UIs. 
For the webpages, mobile UIs, and posters, fixations are spread across the entire upper-left region, while there are two bands of salient regions in desktop UIs: one right above the center of the UI and the other near the upper left-hand corner. 
The most salient area of webpages is around the center-right section of the upper-left quadrant, while that quadrant's uppermost portion attracts the most attention in the mobile UI condition. 
Desktop UIs and posters deviate from this pattern, with the most salient area appearing just above the center of the desktop UIs and posters. 


An omnibus test revealed statistically significant differences
in the average number of fixations per user for the visual content specific to each quadrant (where Q1 = top right, Q2 = top left, Q3 = bottom left, and Q4 = bottom right).
For example, in the general (all-UI-type) condition, $\chi^2(3)\ =\ 183.930, p\ <\ .0001$. %
Similar results were obtained for each specific type of UI.

We then ran Bonferroni-Holm corrected pairwise comparisons in post-hoc testing
and found that the difference between Q1 and Q2 was statistically significant in all cases ($p\ <\ .001$).
The Q1 vs. Q3 difference and the Q1 vs. Q4 one were statistically significant when users viewed the images for three seconds or longer ($p < .001$),
Also, the difference between Q2 and Q3 and that between Q2 and Q4 was statistically significant in all cases ($p\ <\ .001$).
Finally, the Q3 vs. Q4 difference was significant when the viewing time was three seconds or longer ($p\ =\ .018$).




\subsection{Effect of Color}
\label{sec:analysis-color}
\begin{figure*}[!ht]
    \centering
    \def\w{0.28\linewidth}
    \subfloat[All UI types]{
        \begin{minipage}{\w}
            \includegraphics[width=\linewidth]{results/colorhist-img_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results/colorhist-fix-first1s_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results/colorhist-fix-first3s_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results/colorhist-fix_json_color_bias.png}
        \end{minipage}
    }
    \hfill
    \subfloat[Webpage]{
        \begin{minipage}{\w}
            \includegraphics[width=\linewidth]{results_web/colorhist-img_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_web/colorhist-fix-first1s_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_web/colorhist-fix-first3s_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_web/colorhist-fix_json_color_bias.png}
        \end{minipage}
    }
    \hfill
    \subfloat[Desktop UI]{
        \begin{minipage}{\w}
            \includegraphics[width=\linewidth]{results_desktop/colorhist-img_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_desktop/colorhist-fix-first1s_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_desktop/colorhist-fix-first3s_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_desktop/colorhist-fix_json_color_bias.png}
        \end{minipage}
    }
    \\
      \hfill\hspace*{150pt}
    \subfloat[Mobile UI]{
        \begin{minipage}{\w}
            \includegraphics[width=\linewidth]{results_mobile/colorhist-img_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_mobile/colorhist-fix-first1s_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_mobile/colorhist-fix-first3s_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_mobile/colorhist-fix_json_color_bias.png}
        \end{minipage}
    }
    \hfill
    \subfloat[Poster]{
        \begin{minipage}{\w}
            \includegraphics[width=\linewidth]{results_poster/colorhist-img_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_poster/colorhist-fix-first1s_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_poster/colorhist-fix-first3s_json_color_bias.png} \\
            \includegraphics[width=\linewidth]{results_poster/colorhist-fix_json_color_bias.png}
        \end{minipage}
    }
        
    \caption{\REVISION{Color bias -- the 16 most prevalent colors in UIs (top row) 
        and the 16 colors fixated upon most, by frequency, for 
        fixations lasting up to 1\,s (second row), up to 3\,s (third row), and up to 7\,s (bottom row).}}
    \Description{This figure shows the color bias for the overall, webpage, desktop, mobile, and poster, including the color bars for all displayed colors, and the top 16 fixated colors sorted by frequency up to 1 second, 3 seconds, and 7 seconds, respectively.}
    \label{fig:color-bias-results}
\end{figure*}
\begin{figure*}[!ht]
    \centering
    \def\w{0.28\linewidth}
    \subfloat[All UI types]{
        \includegraphics[width=\w]{results/color_bias_brightness_boxplot.pdf}
    }
    \hfill
    \subfloat[Webpage]{
        \includegraphics[width=\w]{results_web/color_bias_brightness_boxplot.pdf}
    }
    \hfill
    \subfloat[Desktop UI]{
        \includegraphics[width=\w]{results_desktop/color_bias_brightness_boxplot.pdf}
    }
    \\
    \phantom{\includegraphics[width=\w]{results_poster/color_bias_brightness_boxplot.pdf}}
    \hfill
    \subfloat[Mobile UI]{
        \includegraphics[width=\w]{results_mobile/color_bias_brightness_boxplot.pdf}
    }
    \hfill
    \subfloat[Poster]{
        \includegraphics[width=\w]{results_poster/color_bias_brightness_boxplot.pdf}
    }
    \hfill
    
   \caption{Color-brightness bias plots comparing the brightness of all the colors displayed and fixated upon. \REVISION{Overall, brighter colors tend to attract slightly more attention than darker ones, especially for short time spans.}}
    
    \Description{This figure shows the color brightness bias for the overall, webpage, desktop, mobile, and poster up to 1 second, 3 seconds, and 7 seconds, respectively.}
    \label{fig:color-brightness-bias-results}
\end{figure*}
We show color bias across different UI types in~\autoref{fig:color-bias-results}. 
The top color bar shows the 16 most prevalent colors in the original UI images for different UI types. The other color bars rank the top 16 colors by the number of fixations on those colors, sorted by frequency.
\REVISION{We computed the 16 most prevalent colors using $k$-means clustering, 
therefore similar colors are merged together.}
	\autoref{fig:color-bias-results} characterizes the color bias across the UI types examined.
The uppermost bar in each pane shows the 16 most prevalent colors in the original UI images, for the relevant UI type. The other bars present those top 16 colors ordered by the frequency of fixations on them.
\REVISION{We computed the 16 most prevalent colors by using $k$-means clustering; 
therefore, similar colors are merged.}
\autoref{fig:color-brightness-bias-results}~compares the colors displayed (``All colors'' in the plots) with those colors receiving fixations.
This comparison of brightness reveals that, on average, brighter colors attract more attention than darker ones. 
Designs for webpages, desktop UIs, and mobile UIs seem to draw greater attention to more brightly colored areas relative to the color mix displayed.  
Posters constitute the only exception: the average brightness value of the colors where fixations occur is lower than that of the colors displayed. 
However, the single color at which participants look most often in posters is still a light one. 
Although desktop UIs' fixation-receiving colors are brighter, on average, than the colors shown overall, the three colors with the largest numbers of fixation points in these UIs are dark ones. 
To investigate further whether a reliable effect exists, we computed the pixel brightness values by using sRGB Luma coefficients (ITU Rec.\,709)~\cite{bezryadin2007luma},
which reflect the corresponding standard chromaticities,
and compared distributions between fixation and non-fixation brightness values.
Bartlett's test of homogeneity of variances was statistically significant 
neither for all UIs combined ($\chi^2(3) = 1.003, p = .8004$) nor for any UI type individually ($\chi^2(3) \leq 0.832, p \geq .8416$).
Therefore, we conclude that color does not significantly affect visual saliency.




\subsection{Saccade Angle and Amplitude}

\begin{figure*}[!ht]
    \centering
    \def\w{0.18\linewidth}
    \subfloat[All UI types]{\includegraphics[width=\w]{figures/scanpath_direction/direction_overall_input.png}} \hfil
    \subfloat[Webpage]{\includegraphics[width=\w]{figures/scanpath_direction/direction_webpage_input.png}} \hfil
    \subfloat[Desktop UI]{\includegraphics[width=\w]{figures/scanpath_direction/direction_desktop_input.png}} \hfil
    \subfloat[Mobile UI]{\includegraphics[width=\w]{figures/scanpath_direction/direction_mobile_input.png}} \hfil
    \subfloat[Poster]{\includegraphics[width=\w]{figures/scanpath_direction/direction_poster_input.png}}
     \caption{Analyzing saccade bias reveals the direction and distance between consecutive fixation points. \REVISION{Gaze directions lead mainly toward the right or bottom portion of the UIs, with the distances being larger near the right -- users prefer moving the gaze from left to right (with larger motions) and from top to bottom.}}
    \Description{This figure shows saccade bias analysis indicating the direction and distance between consecutive fixation points for the overall, webpage, desktop, mobile, and poster.}
    \label{fig:saccade-bias-results}
\end{figure*}
\REVISION{Saccade angle and amplitude reveal the tendency and speed of eye movements. Such data can facilitate optimizing UI elements' placement and the flow of information in a UI. By understanding these metrics, designers can align their designs well with the natural gaze behavior of users, thereby potentially promoting a better user experience.}
\autoref{fig:saccade-bias-results} shows the distributions for the direction and distance 
between two consecutive fixation points, represented by the saccade angle and amplitude in the polar-coordinate system. 
We can see that, overall, user gaze moved mainly towards the right or bottom portion of the UIs.
However, UI types do differ markedly in this respect. 
Users showed a greater preference for left-to-right movement in the webpage condition than with other UI types.
Similarly, users tended to scan posters from left to right, 
with a small number of downward movements, 
but they showed greater variety in the distances by which the gaze moved rightward.
In contrast, users looked both from left to right and from top to bottom when viewing desktop UIs and mobile UIs.
The distances in moves toward the right are larger than those toward the bottom in the desktop condition. 
They remained in about the same range for mobile UI designs.

A Kruskal-Wallis chi-squared test showed statistical significance for all UI types 
({\em e.g.,} $\chi^2(3)\ =\ 484.41,\ p\ <\ .0001$ overall), 
so we ran pairwise comparisons (Bonferroni-Holm corrected) as post-hoc tests,
finding that all directions were significantly different from each other for all UI types;
the rightward direction is the most frequent, followed by motion toward the left, bottom, and \REVISION{top}. 

\subsection{Visited vs. Revisited Elements}

\begin{figure*}[!ht]
    \centering
    \def\w{0.18\linewidth}
    \subfloat[All UI types]{\includegraphics[width=\w]{figures/visited_revisited/_visit_resvisit_overall.png}} \hfil
    \subfloat[Webpage]{\includegraphics[width=\w]{figures/visited_revisited/_visit_resvisit_webpage.png}} \hfil
    \subfloat[Desktop UI]{\includegraphics[width=\w]{figures/visited_revisited/_visit_resvisit_desktop.png}} \hfil
    \subfloat[Mobile UI]{\includegraphics[width=\w]{figures/visited_revisited/_visit_resvisit_mobile.png}} \hfil
    \subfloat[Poster]{\includegraphics[width=\w]{figures/visited_revisited/_visit_resvisit_poster.png}}
    \caption{Visit vs. revisit bias analysis showing the ratios of visited to revisited elements in three element categories. \REVISION{Text elements are more likely than images to be visited and to be revisited.}}
    \Description{This figure shows visit vs. revisit bias analysis showing the ratios of visited and revisited elements in different element categories for the overall, webpage, desktop, mobile, and poster.}
    \label{fig:visit-bias-results}
\end{figure*}

We segmented the UIs and classified the UI elements into three categories -- 
image, text, and face -- by extending the functionality of the UIED model~\cite{xie2020uied}, a model for detecting images and texts on UIs.
Then, we counted the number of elements in each category that were visited (fixated upon) and revisited (fixated upon again).
Once visited, an element is considered revisited if it receives at least three fixation points and the previous fixation was on another element.
The results are shown in~\autoref{fig:visit-bias-results}.
We observed that text elements have a higher fixation probability in our data than images. 
While the dataset's desktop UIs feature many small images (such as icons), which are more prominent than text, 
the opposite was visible in posters: they had large images, typically in a small quantity.
Webpages have about the same number of image and text elements.
It is worth noting that mobile UIs exhibited lower visit and revisit ratios both than other UI types, 
reflecting mobile UIs' reduced opportunities for users returning to the same content later.

We found statistically significant differences in visit and in revisit ratios 
between element types (image, text, and face) for all UI types.
For example, in comparison of the visit ratios for the overall condition, $\chi^2(2)\ =\ 9.295,\ p\ <\ .01$.
Post-hoc pairwise comparisons (Bonferroni-Holm corrected)
revealed statistical significance for all UI types compared.
We conclude that text attracts fixations the most, followed by images and then faces.


	\subsection{Summary}
We can summarize our results thus: %
The upper-left quadrant tends to attract the most fixations, 
while brighter colors do not attract significantly more fixations than \REVISION{less bright} colors. 
As users gaze at UIs, their saccades move mainly from left to right and from top to bottom. 
Participants in our experiment tended to spend more time looking at text elements than images, 
which accounts for the saccade directions' left-to-right tendency. 
\REVISION{Overall, our findings related to mobile UIs are consistent with the results of Leiva et al.~\cite{bruce2005saliency}. When introducing further analysis metrics, we found biases specific to each UI type. The following characteristics and differences emerged, recapped here by UI type:}
\begin{description}
\item[Webpage:] Participants preferred to scan more from left to right when looking at webpages, 
with larger distances between consecutive fixations than they showed with other UI types.
\item[Desktop UI:] Rather than fixations being spread over the top-left quadrant, 
the salient areas of desktop UIs are separated into two areas: right above the center and around the top-left corner. 
\item[Mobile UI:] Mobile UIs exhibit lower visit and revisit ratios than other UI types. 
This indicates that users tend to focus more on a few elements of the UI (the most attractive ones) 
while ignoring others and that there is less likelihood of going back to look at the same elements.
\item[Poster:] In comparison to desktop UIs and mobile UIs, participants demonstrated a much stronger intention to scan from left to right, 
with only a small proportion of saccades being directed from top to bottom. 
The distances between consecutive fixation points show more significant variation here than with other UI types.
\end{description}


==> 05a-Saliency-Prediction.tex <==
\section{Assessing Saliency Map Models}
With the backdrop of the differences identified between UI types, we conducted a comparison among data-driven predictive models for saliency maps.
We considered the state-of-the-art traditional optimization-based model (GBVS) and data-driven models (the SAM and UMSI) alongside improved versions that we developed ourselves, SAM++ and UMSI++.
    \paragraph{Graph-Based Visual Saliency (GBVS)~\cite{harel2006graph}} GBVS is a bottom-up saliency map model for detecting informative features on the basis of the entire image. 
    It employs the saliency-based visual attention model proposed by Itti and Koch~\cite{itti1998model} to extract visual features as computed via linear center-surround operations with Gaussian pyramids for intensity, color, and orientation.
    It then forms graph-based activation maps from visual features and normalizes them to highlight conspicuity. 
    The global visual feature extraction and graph-based activation maps enable the model to capture saliency maps at the global level, which is more efficient than prior approaches relying on local information.
    \paragraph{Saliency Attentive Model (SAM)~\cite{cornia2018predicting, cornia2018sam}} SAM incorporates an attentive convolutional long-short term memory (Attentive ConvLSTM) saliency map model to focus on distinct spatial location features to enhance sequential predictions. 
    The model iteratively and progressively refines the predicted saliency map results via the LSTM architecture. 
    The SAM learns a set of prior maps generated with Gaussian functions to learn saliency priors, such as the center bias typical of human eye fixations, thereby obtaining improved feature-extraction capabilities without needing hand-crafted prior information.
    \paragraph{UMSI~\cite{fosco2020predicting}} UMSI is a unified model of saliency and importance trained on images from several design classes, including posters, infographics, mobile UIs, and natural images.
    It uses an encoder-decoder architecture and aggregates image information at multiple scales to predict visual importance in the input graphic designs. 
    The UMSI employs an automatic classification module for the input graphic designs, to better capture the saliency patterns with class-specific information. 
    It was trained on a dataset for visual importance from cursor-based crowdsourced data.
    Again, while the cursor is a good proxy for eye-tracking, it cannot properly simulate the results captured via data from eye trackers. 
    \paragraph{UMSI++ and SAM++ (Ours)} UMSI++ and SAM++ are variants we created by employing new loss terms and a two-step training process.
The main module of the original UMSI model was trained with KL-divergence~\cite{joyce2011kullback} and Cross-Correlation~\cite{le2007predicting} losses with coefficients 10 and -3. 
The output of the UMSI model is the flipped saliency maps requiring post-processing via black-to-white inversion.
\REVISION{
Our UMSI++ model employs an end-to-end joint training process that entails refining the model via multiple loss terms.
Over the first 10 epochs of training, the model approaches the ground-truth saliency maps by using the Mean Squared Error (MSE) loss 
between the predicted and the ground-truth saliency maps. This helps the model accurately predict the saliency maps.
For the remaining epochs, the model is trained with a combination of loss terms, 
including the KL-divergence and Cross-Correlation loss terms~\cite{le2007predicting} used in the UMSI, 
alongside two additional loss terms: the Normalized Scanpath Saliency (NSS) loss and the Similarity loss. 
The NSS loss quantifies the average normalized saliency at fixation points, 
while the Similarity loss measures the intersection between the predicted and the ground-truth saliency maps. 
These loss terms help the model better capture fixations and improve its overall performance.
Both KL-divergence and Cross-Correlation are distribution-based: they focus on the continuous distributions of the saliency maps, rather than on individual points or locations.
In contrast, NSS and Similarity are location-based in that they focus on the locations of fixation points in the saliency maps. 
Together, these loss terms have been shown to perform well in predicting fixation points, 
and they can help the model better capture eye fixations ~\cite{broda2022individual, zhang2022predicting}.
 Computation details are given in \emph{Supplementary Materials}.
}
The training takes about an hour on one NVIDIA GeForce RTX 2080Ti GPU.
For comparison, we apply the same training pipeline and loss terms to the SAM architecture to get the result for the SAM++ model.



\subsection{Evaluation Metrics}
\label{sec:saliency_metrics}
We evaluated the accuracy by means of six widely applied metrics. 

    \paragraph{Area under ROC Curve (AUC)} AUC is the most commonly used metric for saliency map performance. 
    It evaluates the saliency map as a binary classifier of fixation points at various thresholds. 
    The Receiver Operating Characteristic Curve (ROC Curve) shows the rates of the actual positive points and the false positive ones at multiple discrimination threshold values.  
    AUC is defined as the area under such a curve measuring the true and false positive rates under the binary classifier, which one can compute by taking the integral of the area under the ROC curve in practice.
    AUC-Judd~\cite{judd2009learning, bylinskii2015saliency} is a variation of AUC.
    The true positive rate is defined as the ratio of the number of true positive points to the number of ground-truth fixation points above various threshold values, while the false positive rate is that of the number of false positive points to the total number of non-fixation pixels.
    \paragraph{Normalized Scanpath Saliency (NSS)~\cite{peters2005components}} NSS is the average normalized saliency at fixation points.
    Relative to the AUC metric, NSS is more sensitive in detecting false positive points. 
    The AUC score can be high even when there are many false positive points, given a large number of true positive points -- low-valued false positive points do not affect the AUC score.
    However, all false positive points decrease the normalized saliency value.
    Thus the NSS score penalizes all the false positive points. 
    \paragraph{Information Gain (IG)~\cite{kummerer2014close, kummerer2015information}} IG is used for measuring saliency results beyond systematic bias. 
    \paragraph{Similarity (SIM)~\cite{rubner2000earth, swain1991color}} SIM refers to the intersection between the predicted and the ground-truth saliency maps, thereby indicating the overlapping of the two maps. 
    It is defined as the sum of the minimum value of the normalized predicted saliency map and of the normalized ground-truth map. 
    The similarity score is lower for sparse maps.
    It is sensitive to failed detection of saliency points: the absence of saliency values points to zero similarity, hence reducing the similarity score.
    \paragraph{Pearson's Correlation Coefficient (CC)~\cite{le2007predicting}} CC is employed for evaluating the correlation or dependence between the predicted and the ground-truth saliency maps.
    \paragraph{Kullback-Leibler (KL) Divergence~\cite{joyce2011kullback}} KL Divergence quantifies the difference between the distributions of the saliency map prediction and the ground truth, while the other metrics listed here measure the similarity.

\smallskip 

Computation details are provided in \emph{Supplementary Materials}. The various metrics differ in their sensitivity to false positives or false negatives, what is measured, and the category of metric involved, thus:

\begin{description}
\item [Sensitivity:] All these metrics are sensitive to false negatives, with the KL, IG, and SIM significantly penalizing false negatives, especially when the predicted values are close to zero. 
The normalization step of NSS increases the penalty for detecting false positives and thus makes it more sensitive to false positives than other metrics. The CC is, by definition, a symmetric metric, so it shows equal sensitivity to false positives and false negatives. 
The AUC score is insensitive to false positives -- it can be high even if the resulting saliency maps have many true positives.
\item [Measurement:] The KL measurement assesses dissimilarity while the other metrics gauge similarity.
Accordingly, better models have lower KL scores but higher scores for other metrics.
\item [Metric category:] The location-based metrics (AUC, NSS, and IG) evaluate models in terms of fixation points, while distribution-based ones (SIM, CC, and KL) compute evaluation based on saliency maps as the continuous distribution.
\end{description}



\subsection{Results}
To set a benchmark for saliency maps' prediction, we compared the computational saliency map models qualitatively and quantitatively and judged the predicted location bias. 
We used the dataset's first 52 image blocks (1,872 images) as the training data and the remaining three blocks of images (108 images) for testing. 
All the results shown here come from evaluation with the test data. 

\subsubsection{Qualitative Evaluation}
We present the qualitative comparison of the various models by UI type in~\autoref{fig:saliency_qualitative}. 
For all the models, false positive errors constitute the main kind of error in the results. 
All of them can capture informative areas such as images and text elements, 
but not all of these truly attract the user's attention,
and sometimes, only a small part of an image is considered salient. 
Therefore, it is generally challenging for predictive models to distinguish between informative areas and salient areas. 
Both GBVS and the pretrained UMSI typically capture all image and text areas, which leads to high false positive error levels. 
Models trained on UEyes achieve better results than the pretrained models. 
Our improved model UMSI++ generates the saliency maps that most closely approach the ground-truth fixations,
relative to the other models and across all the UI types. 

\setlength{\tabcolsep}{3pt}
\begin{figure*}[!]
\def\w{0.135\linewidth}
 \centering
\begin{tabular}{c *4c}
& \bf Webpage & \bf Desktop UI & \bf Mobile UI & \bf Poster \\
\bf \begin{turn}{90} 
\ \ \ \ \ \ \ \ \  \begin{tabular}{@{}c@{}}Input \\ Image\end{tabular}
\end{turn} & 
\includegraphics[height=\w]{figures/saliency_qualitative/webpage_input_image.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/desktop_input_image.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/mobile_input_image.jpg} &
\includegraphics[height=\w]{figures/saliency_qualitative/poster_input_image.png} 
\\
\bf \begin{turn}{90} 
\ \ \ \ \ \ \ \  \begin{tabular}{@{}c@{}}Ground \\ Truth\end{tabular}
\end{turn} &
\includegraphics[height=\w]{figures/saliency_qualitative/webpage_ground_truth.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/desktop_ground_truth.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/mobile_ground_truth.jpg} &
\includegraphics[height=\w]{figures/saliency_qualitative/poster_ground_truth.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \ \ \  GBVS 
\end{turn} & 
\includegraphics[height=\w]{figures/saliency_qualitative/webpage_GBVS.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/desktop_GBVS.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/mobile_GBVS.jpg} &
\includegraphics[height=\w]{figures/saliency_qualitative/poster_GBVS.png} 
\\
\bf \begin{turn}{90} 
\ \ \ \ \ \ \begin{tabular}{@{}c@{}}SAM \\ Pretrained\end{tabular}
\end{turn} &
\includegraphics[height=\w]{figures/saliency_qualitative/webpage_SAM_Pretrained.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/desktop_SAM_Pretrained.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/mobile_SAM_Pretrained.jpg} &
\includegraphics[height=\w]{figures/saliency_qualitative/poster_SAM_Pretrained.png} 
\\
\bf \begin{turn}{90} 
\ \ \ \ \  \ \ \ \begin{tabular}{@{}c@{}}SAM \\ on UEyes\end{tabular}
\end{turn} &
\includegraphics[height=\w]{figures/saliency_qualitative/webpage_SAM_UEyes.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/desktop_SAM_UEyes.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/mobile_SAM_UEyes.jpg} &
\includegraphics[height=\w]{figures/saliency_qualitative/poster_SAM_UEyes.png} 
\\
\bf \begin{turn}{90} 
\ \ \ \ \  \ \ \  \begin{tabular}{@{}c@{}}SAM++ \\ on UEyes\end{tabular}
\end{turn} &
\includegraphics[height=\w]{figures/saliency_qualitative/webpage_SAM++_UEyes.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/desktop_SAM++_UEyes.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/mobile_SAM++_UEyes.jpg} &
\includegraphics[height=\w]{figures/saliency_qualitative/poster_SAM++_UEyes.png} 
\\
\bf \begin{turn}{90} 
\ \ \ \  \ \ \begin{tabular}{@{}c@{}}UMSI \\ Pretrained\end{tabular}
\end{turn} &
\includegraphics[height=\w]{figures/saliency_qualitative/webpage_UMSI_pretrained.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/desktop_UMSI_pretrained.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/mobile_UMSI_pretrained.jpg} &
\includegraphics[height=\w]{figures/saliency_qualitative/poster_UMSI_pretrained.png} 
\\
\bf \begin{turn}{90} 
\ \ \ \ \  \ \ \begin{tabular}{@{}c@{}}UMSI \\ on UEyes\end{tabular}
\end{turn} &
\includegraphics[height=\w]{figures/saliency_qualitative/webpage_UMSI_UEyes.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/desktop_UMSI_UEyes.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/mobile_UMSI_UEyes.jpg} &
\includegraphics[height=\w]{figures/saliency_qualitative/poster_UMSI_UEyes.png} 
\\
\bf \begin{turn}{90} 
\ \ \ \ \  \ \ \  \begin{tabular}{@{}c@{}}UMSI++ \\ on UEyes\end{tabular}
\end{turn} &
\includegraphics[height=\w]{figures/saliency_qualitative/webpage_UMSI++_UEyes.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/desktop_UMSI++_UEyes.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/mobile_UMSI++_UEyes.jpg} &
\includegraphics[height=\w]{figures/saliency_qualitative/poster_UMSI++_UEyes.png} 
\\
\end{tabular}
\caption{
    Saliency maps' qualitative comparison. \REVISION{Compared to other models, our improved model UMSI++ generates saliency maps closer to ground truth across all UI types.}
}
\Description{This figure shows qualitative results of different saliency map models for the overall, webpage, desktop, mobile, and poster.}
\label{fig:saliency_qualitative}
\end{figure*}



\subsubsection{Quantitative Comparison across UI Types}

\REVISION{We begin by addressing the importance of training on multiple types of UIs, because training with only one type leads to accuracy reductions with other types. We trained our UMSI++ model on either mobile UI or webpage data from UEyes, respectively, and testing on all UI types used the same test set. Accuracy in predictions for other UI types (those different from what was seen during training) dropped significantly. For example, when the model was trained on mobile UIs, its accuracy fell from 0.899 to 0.844 when it was tested instead on webpages, from 0.890 to 0.803 for desktop UIs, and from 0.924 to 0.849 for posters. Similarly, when the model was trained on webpages, its accuracy decreased from 0.905 to 0.832 for mobile UIs, from 0.890 to 0.813 for desktop UIs, and from 0.924 to 0.848 for posters.
How people perceive visual hierarchies and look at UIs when viewing any given type of UIs could not truly be generalized to other UI types.}

Quantitative comparison of the models as evaluated via the metrics detailed in~\autoref{sec:saliency_metrics} attests that training on UEyes provides both the SAM and the UMSI models with higher accuracy and stronger generalization ability.
Furthermore, our improved model, UMSI++, outperforms the state-of-the-art models by most metrics, as~\autoref{tbl:saliency_quantitative} indicates.
Since AUC is a standard evaluation metric with a range of 0 to 1 for saliency map prediction (where larger values indicate higher accuracy), it lets us quantitatively evaluate and compare the models across UI types graphically in the manner shown in~\autoref{fig:auc_vis}.
The pretrained SAM model performs better than the pretrained UMSI.
However, after training on UEyes, the two perform similarly for all the UI types. 
By introducing new loss terms, UMSI++ achieved the best performance across all the UI types, while SAM++ does did not show greater accuracy than the original SAM trained on UEyes. 
For both SAM and UMSI architectures, the predictions for desktop UIs were the least accurate for every UI type. This is consistent with our observations from the qualitative results.


\begin{table*}[!ht]
\begin{tabular}{l *6c}
\toprule
\textbf{Model} & \textbf{AUC-Judd} $\uparrow$ & \textbf{NSS} $\uparrow$ & \textbf{IG} $\uparrow$ & \textbf{SIM} $\uparrow$ & \textbf{CC} $\uparrow$ & \textbf{KL} $\downarrow$ \\
\midrule
GBVS            & 0.756 $\pm$ 0.104 & 0.256 $\pm$ 0.197 & 3.214 $\pm$ 0.668 & 0.513 $\pm$ 0.097 & 0.314 $\pm$ 0.193 & 3.916 $\pm$ 2.630 \\
SAM Pretrained  & 0.822 $\pm$ 0.074 &  0.377 $\pm$ 0.170 & 3.143 $\pm$ 0.768 & 0.562 $\pm$ 0.081 & 0.522 $\pm$ 0.146 & 2.721 $\pm$ 1.457 \\
SAM on UEyes    & 0.885 $\pm$ 0.057 & \bf 0.434 $\pm$ 0.185 & 3.337 $\pm$ 0.774 & 0.663 $\pm$ 0.081 & 0.720 $\pm$ 0.127 & 2.016 $\pm$ 1.263 \\
SAM++ on UEyes    & 0.868 $\pm$ 0.060 & 0.414 $\pm$ 0.179 & 3.165 $\pm$ 0.774 & 0.666 $\pm$ 0.080 & 0.717 $\pm$ 0.127 & 1.604 $\pm$ 1.185 \\
UMSI Pretrained & 0.778 $\pm$ 0.090 & 0.346 $\pm$ 0.178 & 3.177 $\pm$ 0.796 & 0.521 $\pm$ 0.078 & 0.431 $\pm$ 0.155 & 3.757 $\pm$ 1.769 \\
UMSI on UEyes   & 0.878 $\pm$ 0.066 & 0.424 $\pm$ 0.187 & \bf 3.376 $\pm$ 0.807 & 0.639 $\pm$ 0.085 & 0.699 $\pm$ 0.156 & 2.676 $\pm$ 1.408 \\
UMSI++ on UEyes & \bf 0.905 $\pm$ 0.044 & 0.401 $\pm$ 0.173 & 3.320 $\pm$ 0.744 & \bf 0.733 $\pm$ 0.069 & \bf 0.833 $\pm$ 0.078 & \bf 1.166 $\pm$ 0.772 \\
\bottomrule
\end{tabular}
\caption{
    Saliency maps' quantitative evaluation, with mean $\pm$ SD reported for each metric.
    Arrows indicate the direction of the importance; e.g., $\uparrow$ means ``higher is better''.
    The best result in each column is presented in bold.
    \REVISION{UMSI++ outperforms the other models for most evaluation metrics.}
}
\Description{This table shows quantitative saliency maps results of different models on the mentioned metrics for the overall, webpage, desktop, mobile, and poster.}
\label{tbl:saliency_quantitative}
\end{table*}


\setlength{\tabcolsep}{0pt}
\def\arraystretch{1}%
\begin{figure*}[!]
\def\w{0.22\linewidth}
 \centering
\begin{tabular}{*4c}
\bf \ \ \  \ \ \ \ \ \  GBVS & \bf \ \ \  \ \ \ \ \ \ SAM Pretrained  & \bf \ \ \  \ \ \ \ \ \ SAM on UEyes  & \bf \ \ \  \ \ \ \ \ \ SAM++ on UEyes     \\
\includegraphics[width=\w]{figures/saliency_quantitative/AUC_GBVS.png} &
\includegraphics[width=\w]{figures/saliency_quantitative/AUC_SAM_Pretrained.png} &
\includegraphics[width=\w]{figures/saliency_quantitative/AUC_SAM_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_quantitative/AUC_SAM++_UEyes.png} \\
   & \bf \ \ \ \ \ \ \ \ \ UMSI Pretrained  & \bf \ \ \ \ \ \ \ \ \  UMSI on UEyes  & \bf \ \ \ \ \ \ \ \ \  UMSI++ on UEyes     \\
 & \includegraphics[width=\w]{figures/saliency_quantitative/AUC_UMSI_Pretrained.png} &
\includegraphics[width=\w]{figures/saliency_quantitative/AUC_UMSI_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_quantitative/AUC_UMSI++_UEyes.png} \\
\end{tabular}
\caption{
Comparison of saliency map models' predictive accuracy, with AUC-Judd (designed to measure saliency map performance) as the metric. Larger values indicate higher accuracy. The figure shows that UMSI++ performs best across all the UI types.
}
\Description{This figure shows the AUC metric results of different models on the mentioned metrics for the overall, webpage, desktop, mobile, and poster.}
\label{fig:auc_vis}
\end{figure*}


\subsubsection{Predicted Location Bias}

	\autoref{fig:saliency_bias} presents a visualization of the location bias of the saliency maps predicted by the various models considered.
All models except GBVS can capture the upper-left location bias identified for UIs. 
The models trained on our UEyes dataset can capture that location bias more accurately than the pretrained ones.
After training with UEyes, the SAM, SAM++, and UMSI models achieved similar results for saliency location bias. 
Our improved model displays the greatest similarity to the ground truth for location bias.
It is clearly evident from the visualization that all the models over-capture the salient areas and produce many false positive errors, which aligns with what we found in the qualitative comparison. 
Saliency is tricky to detect for mapping predictions in contexts of webpages and (especially) desktop UIs.
Salient areas are spread more sparsely in the upper-left quadrant of webpages than in other UI types. 
The salient portions of desktop UIs are separated into the two sub-areas mentioned earlier on, one right above the center line and the other near the top left. 
It is far more challenging for the models to simulate sparser areas. 
Still, the models trained on UEyes capture such sparse salient areas better, while other models can only capture the entire areas, with many more false positives. 
All of the models except GBVS can capture the most salient parts of mobile UI designs (the upper-left quadrant) and posters (right above the center) well. 
The ones trained on UEyes are similarly accurate in their location bias results across webpages, desktop UIs, and mobile UIs; 
however, UMSI++ reveals the location bias connected with posters better than the other models do, thanks to its detection of lower saliency at the top of posters. 

\setlength{\tabcolsep}{1pt}
\def\arraystretch{1}%
\begin{figure*}[!]
\def\w{0.15\linewidth}
 \centering
\begin{tabular}{c *5c}
& \bf All UI types & \bf Webpage & \bf Desktop UI & \bf Mobile UI & \bf Poster \\
\bf \begin{turn}{90} 
\ \ \ \ \ \ \ \ \ \  \begin{tabular}{@{}c@{}}Ground \\ Truth\end{tabular}
\end{turn} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_overall_bias_Ground_Truth.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_webpage_bias_Ground_Truth.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_desktop_bias_Ground_Truth.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_mobile_bias_Ground_Truth.png}  &
\includegraphics[width=\w]{figures/saliency_bias/normalized_poster_bias_Ground_Truth.png} 
\\ 
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \ \ \ \ \  GBVS 
\end{turn} & 
\includegraphics[width=\w]{figures/saliency_bias/normalized_overall_bias_GBVS.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_webpage_bias_GBVS.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_desktop_bias_GBVS.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_mobile_bias_GBVS.png}  &
\includegraphics[width=\w]{figures/saliency_bias/normalized_poster_bias_GBVS.png}
\\
\bf \begin{turn}{90} 
\ \ \ \ \ \ \ \begin{tabular}{@{}c@{}}SAM \\ Pretrained\end{tabular}
\end{turn} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_overall_bias_SAM_Pretrained.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_webpage_bias_SAM_Pretrained.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_desktop_bias_SAM_Pretrained.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_mobile_bias_SAM_Pretrained.png}  &
\includegraphics[width=\w]{figures/saliency_bias/normalized_poster_bias_SAM_Pretrained.png}
\\
\bf \begin{turn}{90} 
\ \ \ \ \ \ \ \ \  \begin{tabular}{@{}c@{}}SAM \\ on UEyes\end{tabular}
\end{turn} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_overall_bias_SAM_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_webpage_bias_SAM_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_desktop_bias_SAM_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_mobile_bias_SAM_UEyes.png}  &
\includegraphics[width=\w]{figures/saliency_bias/normalized_poster_bias_SAM_UEyes.png}
\\
\bf \begin{turn}{90} 
\ \ \ \ \ \ \ \ \ \begin{tabular}{@{}c@{}}SAM++ \\ on UEyes\end{tabular}
\end{turn} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_overall_bias_SAM++_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_webpage_bias_SAM++_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_desktop_bias_SAM++_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_mobile_bias_SAM++_UEyes.png}  &
\includegraphics[width=\w]{figures/saliency_bias/normalized_poster_bias_SAM++_UEyes.png}
\\
\bf \begin{turn}{90} 
\ \ \ \ \ \ \ \ \begin{tabular}{@{}c@{}}UMSI \\ Pretrained\end{tabular}
\end{turn} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_overall_bias_UMSI_Pretrained.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_webpage_bias_UMSI_Pretrained.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_desktop_bias_UMSI_Pretrained.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_mobile_bias_UMSI_Pretrained.png}  &
\includegraphics[width=\w]{figures/saliency_bias/normalized_poster_bias_UMSI_Pretrained.png}
\\
\bf \begin{turn}{90} 
\ \ \ \ \ \ \ \ \ \ \begin{tabular}{@{}c@{}}UMSI \\ on UEyes\end{tabular}
\end{turn} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_overall_bias_UMSI_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_webpage_bias_UMSI_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_desktop_bias_UMSI_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_mobile_bias_UMSI_UEyes.png}  &
\includegraphics[width=\w]{figures/saliency_bias/normalized_poster_bias_UMSI_UEyes.png}
\\
\bf \begin{turn}{90} 
\ \ \ \ \ \ \ \ \ \begin{tabular}{@{}c@{}}UMSI++ \\ on UEyes\end{tabular}
\end{turn} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_overall_bias_UMSI++_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_webpage_bias_UMSI++_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_desktop_bias_UMSI++_UEyes.png} &
\includegraphics[width=\w]{figures/saliency_bias/normalized_mobile_bias_UMSI++_UEyes.png}  &
\includegraphics[width=\w]{figures/saliency_bias/normalized_poster_bias_UMSI++_UEyes.png}
\\
\end{tabular}
\vspace{-15px}
\caption{
    Comparison of the location bias of saliency maps predicted by different models across UI types. \REVISION{UMSI++ shows the greatest similarity to the ground-truth location bias.}
}
\Description{This figure shows the location bias of saliency maps predicted by different models for the overall, webpage, desktop, mobile, and poster.}
\label{fig:saliency_bias}
\end{figure*}


==> 05b-Scanpath-Prediction.tex <==
\section{Assessing Scanpath Models}
In scanpath prediction, the goal is to predict a sequence of fixations. 
The problem is much more challenging than that of saliency maps because the order of the fixations must be retained.
Below, we report on how well computational models fared with the four UI types, from a 
comparison of four models:
    \paragraph{Itti-Koch-based model~\cite{itti1998model}} The Itti-Koch-based model is a model proposed in the pre-deep-learning era. 
    It generates a saliency map by extracting visual features for intensity, color, and orientation through a set of linear center-surround operations, 
    then employs a ``winner-takes-all'' strategy to select the attended position. %
    The model repeatedly applies inhibition of return feedback to inhibit the chosen position in the saliency map and, thereby, arrive at the resulting scanpath.
    \paragraph {DeepGaze III ~\cite{kummerer2022deepgaze}} DeepGaze III predicts the sequence of fixation points in scanpaths over static images. 
    It takes both the input image and the positions of the previous four fixation points to predict the density/probabilistic map for the next fixation point. 
    After that, it generates the scanpath by recursively selecting the next fixation point with the highest probability value from the density map and adding the new predicted fixation point to infer the density map for the next point. 
    DeepGaze III's method concentrates on applying fixation point detection to form the final scanpath. 
    \paragraph {DeepGaze++ (Ours)} DeepGaze++ offers an alternative. Although DeepGaze III can take the information of previous fixation points to generate the density of the next point, it often arrives at similar density maps for consecutive fixation point predictions. 
    In the proposed modification, we repeatedly select the position with the highest probability from the density map and apply inhibition of return to inhibit the chosen position in the saliency map. %
    For the $i$th previous fixation point's information, we assign a weight of $1 - 0.1 \cdot (i-1)$ to the inhibition of return feedback so that older fixation points have less effect on the prediction results.
    \paragraph{PathGAN~\cite{Assens2018pathgan}} PathGAN is a deep convolutional-recurrent neural network trained on adversarial examples. 
    The generator takes the image as input to generate the corresponding scanpath. 
    The discriminator encodes both the image and the scanpath to ascertain whether a scanpath is realistic for a given image. 
    This enables PathGAN to generate more realistic scanpaths. 
    However, it focuses exclusively on the path and cannot predict fixation points.
    \REVISION{\paragraph {PathGAN++ (Ours)} The PathGAN model can generate more accurate trajectories for scanpaths than other models, but we can increase the scanpaths' accuracy still further to have PathGAN++ by adding a Dynamic Time Warping (DTW) %
loss term that maximizes the similarity between the predicted scanpath and the ground truth in temporal order.} 

\subsection{Evaluation Metrics}
\label{sec:scanpath_metrics}
We used six metrics, measuring various properties, to evaluate the scanpath models. \REVISION{All are commonly applied for scanpath evaluation~\cite{anderson2015comparison, fahimi2021metrics}, with the first three described below seeing the most frequent use in this field, since they capture the temporal and spatial aspects of visual attention. The final three metrics were employed for completeness.}
    \paragraph{Dynamic Time Warping (DTW)} DTW is a standard metric for similarity between two temporal sequences, of different lengths~\cite{berndt1994using, salvador2007toward}.
    The DTW metric finds the optimal match and computes the distance for two scanpaths monotonically without missing essential features. %
    \paragraph{Time Delay Embedding (TDE)} TDE creates the sets of time-delay embedding vectors for the predicted and the ground-truth scanpaths by collecting all the consecutive subscanpaths of a given length as vectors~\cite{tim1991embedology, wang2011simulating}. %
    We look for the vector from the predicted scanpath for each time-delay embedding vector from the ground-truth scanpath with the minimal distance. 
    Thus, TDE measures the differences between subscanpaths to evaluate the scanpaths.
    \paragraph{Eyenalysis} Eyenalysis performs a double mapping between two scanpaths~\cite{mathot2012eyenalysis}:
    for each fixation point along one scanpath, the procedure finds the spatially closest fixation point on the other scanpath, and then
    it performs the same procedure the other way around. 
    Eyenalysis measures the average distances for all the closest pairs found.
    \paragraph{Cross-Recurrence (REC)} REC involves measuring the matching ratio of fixation points within the two scanpaths~\cite{zbilut2006recurrence}. %
    To use this metric, we truncate the two scanpaths to the same length, that of the shorter of the two scanpaths. 
    Then, we define fixation pairs whose distance is below a certain threshold value as recurrences (we set the threshold to be the image size scaled by 0.05).
    The REC process counts the recurrences and computes the percentage of recurrences out of all the fixation pairs on the two scanpaths.
    \paragraph{Weighted Determinism (DET)} DET is the percentage of recurrent fixation points on subscanpaths in which all the pairs of corresponding fixation points are recurrences and all such recurrent fixation point pairs contain different fixation points from both scanpaths~\cite{anderson2015comparison, fahimi2021metrics}. 
    In its original formulation, the Determinism metric~\cite{anderson2015comparison} produces only the number of corresponding subscanpaths. %
    We propose computing their percentage, to measure the subscanpaths better.
    \paragraph{Center of Recurrence Mass (CORM)} CORM refers to the distance between the center of recurrences, thus indicating the dominant lag of recurrences~\cite{anderson2015comparison, fahimi2021metrics}. %
    The CORM score is lower when the recurrent fixation point pairs on the scanpaths are closer in time. 



\smallskip 

Whereas DTW, TDE, and Eyenalysis measure fixations' position and sequence in temporal order as they match the two sequences differently, 
REC and DET measure only the similarity of fixation positions.
They have higher values if the fixation points in the two sequences are close, irrespective of the temporal order. 
The CORM measurement serves to detect the dominant lag of recurrences. %



\subsection{Results}



\subsubsection{Qualitative Evaluation}

Our qualitative comparison of the various models across UI types is depicted in~\autoref{fig:scanpath_qualitative}. 
Overall, the models cannot predict results accurately relative to the ground-truth data. 
The pretrained PathGAN model and the DeepGaze III model get stuck in local areas, so the predicted points end up in clusters. 
Because of the similar density maps predicted by DeepGaze III for consecutive fixation points, that model selects positions for fixation points that are nearby, thereby producing a cluster of points and getting ``bogged down'' in that cluster.
PathGAN can only generate the scanpath, without considering fixation points.
Therefore, it is impossible to infer which points users give more visual attention from the PathGAN results. 
The Itti-Koch-based model, PathGAN trained on UEyes, DeepGaze++, and PathGAN++ show better prediction results.
\REVISION{That said, most scanpaths predicted by PathGAN and PathGAN++ trained on UEyes are biased to be around the center of the UIs. Also, all the models tend to predict scanpaths with many fixation points, not all of them in salient areas.}

\setlength{\tabcolsep}{2pt}
\def\arraystretch{1}%
\begin{figure*}[!]
\def\w{0.15\linewidth}
\def\ww{0.155\linewidth}
 \centering
\begin{tabular}{c *4c}
& \bf Webpage & \bf Desktop UI & \bf Mobile UI & \bf Poster \\
\bf \begin{turn}{90} 
  \bf \ \ \ \ \ \  Input Image
\end{turn} & 
\includegraphics[height=\w]{figures/saliency_qualitative/webpage_input_image.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/desktop_input_image.png} &
\includegraphics[height=\w]{figures/saliency_qualitative/mobile_input_image.jpg} &
\includegraphics[height=\w]{figures/saliency_qualitative/poster_input_image.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \   \REVISION{Ground Truth}
\end{turn} &
\includegraphics[height=\w]{figures/scanpath_qualitative/webpage_ground_truth.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/desktop_ground_truth.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/mobile_ground_truth.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/poster_ground_truth.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \REVISION{Itti-Koch-based}
\end{turn} & 
\includegraphics[height=\w]{figures/scanpath_qualitative/webpage_Itti_Koch.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/desktop_Itti_Koch.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/mobile_Itti_Koch.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/poster_Itti_Koch.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \REVISION{\begin{tabular}{@{}c@{}}DeepGaze III \\ Pretrained\end{tabular}}
\end{turn} & 
\includegraphics[height=\w]{figures/scanpath_qualitative/webpage_DeepGazeIII.png} &
\includegraphics[height=\ww]{figures/scanpath_qualitative/desktop_DeepGazeIII.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/mobile_DeepGazeIII.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/poster_DeepGazeIII.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \REVISION{ DeepGaze++}
\end{turn} & 
\includegraphics[height=\w]{figures/scanpath_qualitative/webpage_DeepGaze++.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/desktop_DeepGaze++.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/mobile_DeepGaze++.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/poster_DeepGaze++.png} 
\\
\bf \begin{turn}{90} 
\ \ \ \ \ \  \REVISION{\begin{tabular}{@{}c@{}}PathGAN \\ Pretrained\end{tabular}}
\end{turn} & 
\includegraphics[height=\w]{figures/scanpath_qualitative/webpage_PathGAN_Pretrained.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/desktop_PathGAN_Pretrained.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/mobile_PathGAN_Pretrained.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/poster_PathGAN_Pretrained.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \  \ \ \ \ \ \REVISION{\begin{tabular}{@{}c@{}}PathGAN \\ on UEyes\end{tabular}}
\end{turn} & 
\includegraphics[height=\w]{figures/scanpath_qualitative/webpage_PathGAN_UEyes.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/desktop_PathGAN_UEyes.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/mobile_PathGAN_UEyes.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/poster_PathGAN_UEyes.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \ \REVISION{\begin{tabular}{@{}c@{}}PathGAN++ \\ on UEyes\end{tabular}}
\end{turn} & 
\includegraphics[height=\w]{figures/scanpath_qualitative/webpage_PathGAN++.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/desktop_PathGAN++.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/mobile_PathGAN++.png} &
\includegraphics[height=\w]{figures/scanpath_qualitative/poster_PathGAN++.png} 
\\
\end{tabular}
\vspace{-10px}
\caption{
    Scanpaths' qualitative comparison. 
    \REVISION{DeepGaze++ can predict fixation points better but cannot predict realistic scanpaths. PathGAN++ is able to predict a realistic trajectory but not accurate fixation points. %
Trajectories' first portion is presented in blue, and their end in black (color gradient). The starting point is highlighted with a red border.}
}
\Description{This figure shows qualitative results of different scanpath models for the overall, webpage, desktop, mobile, and poster.}
\label{fig:scanpath_qualitative}
\end{figure*}

\subsubsection{Quantitative Evaluation}
\autoref{tbl:scanpaths_quantitative} presents how the models stack up by each of the evaluation metrics outlined in~\autoref{sec:scanpath_metrics}. %
\REVISION{For a fair comparison, since these metrics depend on the scanpath length, we made sure that the predicted scanpaths generated by all the models have exactly 15 fixation points.}
Since DTW is a standard metric for scanpaths' evaluation (where smaller values indicate higher accuracy), we can elaborate on our comparison of the models across UI types in the manner shown in~\autoref{fig:dtw_vis}.
For all models apart from the Itti-Koch-based one, desktop UIs have higher DTW values, indicating lower accuracy of the predicted values than seen with other UI types: scanpaths in desktop UI conditions are harder to predict. All of the models are at their best with mobile UIs.
DeepGaze III was the worst-performing model for all UI types except mobile UIs. 
 \REVISION{The PathGAN++ model shows superior performance in comparison to the other models by the DTW, TDE, and Eyenalysis metrics. This is a testament to our model's ability to simulate real scanpath trajectories.
 However, the results are still qualitatively inaccurate. %
 We can conclude, then, that the metrics currently applied for evaluating scanpaths may not be sufficient to capture the more nuanced aspects of eye movements. 
 } 

\begin{revision}
\subsubsection{Comparison between PathGAN++ and DeepGaze++}

Comparing the performance of PathGAN++ and DeepGaze++ reveals that each model has its own strengths and limitations.
Though PathGAN++ excels at generating realistic trajectories by dint of the discriminative component in the model architecture, 
it falls short in predicting proper fixation points, and the points generated often lie outside the areas of interest.
DeepGaze++, on the other hand, is better at predicting fixation points, since its operation is based on saliency maps that highlight elements in the UIs. However, it can suffer from repetitive density maps for consecutive fixation point predictions, leading to unrealistic scanpaths. Additionally, the mechanism for inhibition of return is deterministic and not differentiable, so it cannot be optimized by means of any loss terms. This trait can hamper its optimization.
\end{revision}




\begin{revision}
\begin{table*}[!ht]
\begin{tabular}{l *7c}
\toprule
\textbf{Model} & \textbf{DTW} $\downarrow$ & \textbf{TDE} $\downarrow$ & \textbf{Eyenalysis} $\downarrow$ & \textbf{REC} $\uparrow$ & \textbf{DET} $\uparrow$ & \textbf{CORM} $\downarrow$ \\
\midrule
Itti-Koch-based &   6.282 $\pm$ 0.973 &   0.147 $\pm$ 0.027 &     0.043 $\pm$ 0.022 & 2.224 $\pm$ 2.053 & 2.021 $\pm$ 10.854 & 34.497 $\pm$ 22.890 \\ 
DeepGaze III Pretrained   &  7.650 $\pm$ 2.899  & 0.250 $\pm$ 0.078  &  0.124 $\pm$ 0.072 &  1.290 $\pm$ 3.281 &  1.025 $\pm$ 8.510  &  \bf 13.838  $\pm$ 24.082 \\ 
DeepGaze++  &  5.230  $\pm$ 1.180 & 0.133  $\pm$ 0.031 & \bf 0.043  $\pm$ 0.022 & 1.876  $\pm$ 1.700 & 1.778  $\pm$ 10.046  & 31.590  $\pm$ 23.120 \\
\REVISION{PathGAN Pretrained}    &     4.381 $\pm$ 1.559 &    0.160 $\pm$ 0.054 &    0.072 $\pm$ 0.036 & \bf 3.896 $\pm$ 5.049 &  \bf 7.039 $\pm$ 18.651 & 22.528 $\pm$ 22.970 \\ 
\REVISION{PathGAN on UEyes}         &  4.354 $\pm$ 1.322 &   0.121 $\pm$ 0.040 &   0.045 $\pm$ 0.024 & 2.414 $\pm$ 2.455 &  5.687 $\pm$ 17.960 & 27.613 $\pm$ 21.644   \\ 
\REVISION{PathGAN++ on UEyes}   &   \bf  4.236 $\pm$ 1.332 &    \bf 0.120 $\pm$ 0.041 &  \bf  0.043 $\pm$ 0.022 &   2.810 $\pm$ 2.743 &  5.761 $\pm$ 16.053 & 27.956 $\pm$ 21.544 \\ 
\bottomrule
\end{tabular}
\caption{Evaluation of scanpaths, with the mean $\pm$ SD reported for each metric. 
   Arrows denote the direction of the importance; e.g., $\uparrow$ means ``higher is better.''
    Each column's best result is highlighted in boldface.
    \REVISION{PathGAN++ outperforms the other models by all three metrics applied for measuring the fixation sequence in temporal order (DTW, TDE, and Eyenalysis).}
}
\Description{This table shows quantitative results of different scanpath models on the mentioned scanpath evaluation metrics for the overall, webpage, desktop, mobile, and poster.}
\label{tbl:scanpaths_quantitative}
\end{table*}
\end{revision}

\setlength{\tabcolsep}{0pt}
\def\arraystretch{1}%
\begin{figure*}[!]
\def\w{0.166\linewidth}
 \centering
\begin{tabular}{*6c}
\bf \ \ \ \ \ \ Itti-Koch-based &  \bf \ \ \  \ \ \ \  \begin{tabular}{@{}c@{}}DeepGaze III \\ Pretrained \end{tabular} & \ \  \ \ \ \ \bf DeepGaze++   & \bf \ \ \   \ \ \REVISION{\begin{tabular}{@{}c@{}}PathGAN \\ Pretrained\end{tabular}} & \bf  \ \ \ \ \ \REVISION{\begin{tabular}{@{}c@{}}PathGAN \\ on UEyes\end{tabular}}  & \bf  \ \ \  \ \ \REVISION{\begin{tabular} {@{}c@{}}PathGAN++ \\ on UEyes\end{tabular}}  \\
\includegraphics[width=\w]{figures/scanpath_quantitative/DTW_Itti-Koch-based.png} &
\includegraphics[width=\w]{figures/scanpath_quantitative/DTW_DeepGazeIII.png} &
\includegraphics[width=\w]{figures/scanpath_quantitative/DTW_DeepGaze++.png} &
\includegraphics[width=\w]{figures/scanpath_quantitative/DTW_PathGAN_Pretrained.png} &
\includegraphics[width=\w]{figures/scanpath_quantitative/DTW_PathGAN_UEyes.png} &
\includegraphics[width=\w]{figures/scanpath_quantitative/DTW_PathGAN++.png} \\
\end{tabular}
\vspace{-15pt}
\caption{
Comparison of predictive accuracy for scanpath models, with DTW as the metric \REVISION{(measuring the fixation sequence in temporal order)}. Smaller values indicate higher accuracy. The figure shows that DeepGaze++ performs best, across all UI types. %
}
\Description{This figure shows the dynamic time warping (DTW) metric results of different models on the mentioned metrics for the overall, webpage, desktop, mobile, and poster.}
\label{fig:dtw_vis}
\end{figure*}


\subsubsection{Saccade Angle and Amplitude Distribution}

\autoref{fig:predict_saccade_direction} characterizes the saccade-angle and amplitude-distribution aspect of our comparison.
None of the models can capture the same distributions as the ground-truth data. 
Human saccade directions are primarily from left to right, with a small proportion of motions from top to bottom. 
The pretrained PathGAN model and DeepGaze III have clustered distributions due to the ``stuck points'' on the predicted scanpaths. %
\REVISION{PathGAN trained on UEyes and PathGAN++ both display an incorrect center bias to the distribution.}
Furthermore, the inhibition of return implemented in the Itti-Koch-based model and DeepGaze++ avoids small distances between consecutive fixation points.
Hence, the saccade amplitudes are more significant than in the ground truth. 
We found that most saccade directions predicted by DeepGaze++ are rightward ones for desktop UIs, mobile UIs, and posters, which demonstrates that DeepGaze++ can capture the actual tendencies visible with these UI types. 
However, it is still incorrect for webpages and cannot predict the gaze's tendency to move toward the bottom of the UIs. 

\setlength{\tabcolsep}{1.5pt}
\def\arraystretch{1}%
\begin{figure*}[!]
\def\w{0.18\linewidth}
 \centering
\begin{tabular}{c *5c}
& \bf \ \ \ \ All UI types & \bf \ \ \ \ Webpage & \bf \ \ \ \ \ \ \ \ Desktop UI & \bf \ \ \ \ \ \  Mobile UI & \bf \ \ \ Poster \\
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \  \ \ \   Ground Truth
\end{turn} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_overall_ground_truth.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_webpage_ground_truth.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_desktop_ground_truth.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_mobile_ground_truth.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_poster_ground_truth.png} 
\\
\bf \begin{turn}{90} 
\bf \ \  \ \ \  Itti-Koch-based
\end{turn} & 
\includegraphics[width=\w]{figures/scanpath_direction/direction_Itti-Koch-based_overall.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_Itti-Koch-based_webpage.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_Itti-Koch-based_desktop.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_Itti-Koch-based_mobile.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_Itti-Koch-based_poster.png} 
\\
\bf \begin{turn}{90} 
 \ \ \ \  \ \ \ \begin{tabular}{@{}c@{}}DeepGaze III \\ Pretrained\end{tabular}
\end{turn} & 
\includegraphics[width=\w]{figures/scanpath_direction/direction_DeepGazeIII_overall.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_DeepGazeIII_webpage.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_DeepGazeIII_desktop.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_DeepGazeIII_mobile.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_DeepGazeIII_poster.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \  \ \ DeepGaze++
\end{turn} & 
\includegraphics[width=\w]{figures/scanpath_direction/direction_DeepGaze++_overall.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_DeepGaze++_webpage.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_DeepGaze++_desktop.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_DeepGaze++_mobile.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_DeepGaze++_poster.png} 
\\
\bf \begin{turn}{90} 
 \ \ \ \ \ \ \   \ \ \  \REVISION{\begin{tabular}{@{}c@{}}PathGAN \\ Pretrained\end{tabular}}
\end{turn} & 
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN_Pretrained_overall.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN_Pretrained_webpage.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN_Pretrained_desktop.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN_Pretrained_mobile.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN_Pretrained_poster.png} 
\\
\bf \begin{turn}{90} 
 \ \ \ \ \ \ \ \   \ \ \  \REVISION{\begin{tabular}{@{}c@{}}PathGAN \\ on UEyes\end{tabular}}
\end{turn} & 
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN_UEyes_overall.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN_UEyes_webpage.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN_UEyes_desktop.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN_UEyes_mobile.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN_UEyes_poster.png} 
\\
\bf \begin{turn}{90} 
 \ \ \ \ \ \  \ \ \  \REVISION{\begin{tabular}{@{}c@{}}PathGAN++ \\ on UEyes\end{tabular}}
\end{turn} & 
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN++_overall.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN++_webpage.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN++_desktop.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN++_mobile.png} &
\includegraphics[width=\w]{figures/scanpath_direction/direction_PathGAN++_poster.png} 
\\
\end{tabular}
\caption{
    Distributions of saccade angles and amplitudes compared across scanpath-based predictive models. \REVISION{Human saccade %
directions are primarily left-to-right, with a small proportion being from top to bottom. None of the models can capture the same distributions as the ground-truth data.}  
}
\Description{This figure shows the saccade angle and amplitude distribution comparison for scanpath predictive models for the overall, webpage, desktop, mobile, and poster.}
\label{fig:predict_saccade_direction}
\end{figure*}

 
\subsubsection{Visited and Revisited Elements}
Our comparison of visited- and revisited-element ratios for the various models is described in~\emph{Supplementary Materials}.
All the models can correctly predict that text elements are more likely to receive fixations than images are. 
The pretrained PathGAN model and DeepGaze III underestimate the visiting and revisiting ratios both. 
DeepGaze++ displays the best prediction for the former but overestimates the revisit ratios for all UI types.
All the models reflect the fact that both ratios are lower with mobile UIs than with other UI types.
Still, every model except DeepGaze++ underestimates the visiting and the revisiting ratio for this type of UI.
Most models' predictions for element visit and revisit ratios are the closest to the ground truth in the case of poster designs.
\REVISION{PathGAN++ is the model that yields the predictions closest to the ground truth for visiting and revisiting of elements, with the exception of its underestimation for mobile UIs.}






==> Makefile <==
# This Makefile allows to compile the paper in a temp dir, to avoid syncing autogenerated files in Dropbox.

PAPER = main

BIBFILE = Reference.bib
BSTFILE = ACM-Reference-Format.bst

CURDIR = "$(shell pwd)"
OUTDIR = /tmp/saliency

all: dirs paper bibs
	$(MAKE) bibs
	$(MAKE) paper

dirs:
	mkdir -p $(OUTDIR)

paper: dirs $(wildcard *.tex)
	pdflatex -output-directory $(OUTDIR) $(PAPER).tex

bibs: paper
	cd $(OUTDIR); ln -sf $(CURDIR)/$(BIBFILE) .; \
	              ln -sf $(CURDIR)/$(BSTFILE) .; \
	              bibtex $(PAPER).aux; \
	              cd -

clean: dirs
	cd $(OUTDIR); rm -f *.log *.blg *.bbl *.out *.aux \
	                    *.bcf *.toc *.spl *.tpt *.synctex.gz *.run.xml; \
	              cd -

